Machine Learning based IoT Edge Node Security Attack and Countermeasures

Advances in technology have enabled tremendous progress in the development of a highly connected ecosystem of ubiquitous computing devices collectively called the Internet of Things (IoT). Ensuring the security of IoT devices is a high priority due to the sensitive nature of the collected data. Physically Unclonable Functions (PUFs) have emerged as critical hardware primitive for ensuring the security of IoT nodes. Malicious modeling of PUF architectures has proven to be difficult due to the inherently stochastic nature of PUF architectures. Extant approaches to malicious PUF modeling assume that a priori knowledge and physical access to the PUF architecture is available for malicious attack on the IoT node. However, many IoT networks make the underlying assumption that the PUF architecture is sufficiently tamper-proof, both physically and mathematically. In this work, we show that knowledge of the underlying PUF structure is not necessary to clone a PUF. We present a novel non-invasive, architecture independent, machine learning attack for strong PUF designs with a cloning accuracy of 93.5% and improvements of up to 48.31% over an alternative, two-stage brute force attack model. We also propose a machine-learning based countermeasure, discriminator, which can distinguish cloned PUF devices and authentic PUFs with an average accuracy of 96.01%. The proposed discriminator can be used for rapidly authenticating millions of IoT nodes remotely from the cloud server.

==> 0_abstract.tex <==
\begin{abstract}
Physically Unclonable Functions (PUFs) are security primitives that can generate a unique digital signature by exploiting intrinsic differences in the physical properties of an integrated circuit. 
However, the advent of machine learning models have enabled attacks on the Challenge-Response Protocol that use strong PUFs for authentication. 
These attacks typically assume that the underlying architecture of the target PUF is known and leverage other information gleaned through invasive attacks, such as side-channel attacks, to mathematically model the inherent characteristics of the target PUF. 
Our work shows that knowledge of the underlying PUF structure is not necessary to clone a PUF. We present a novel non-invasive, architecture independent, machine learning attack for strong PUF designs with a cloning accuracy of 93.5\% and  improvements of up to 48.31\% over an alternative, two-stage brute force attack model. 
We also propose a machine-learning based countermeasure, \textit{discriminator}, which can distinguish cloned PUF devices and authentic PUFs with an average accuracy of 96.01\%.
\end{abstract}


==> 1_intro.tex <==
\section{Introduction}
Given the extent to which electronic devices are integrated into our daily lives, adversarial attacks on such devices can lead to high levels of security and trust issues. 
Classical cryptography allows for security for such devices through obfuscation of a secret binary key, an important piece of information that is unknown to an adversary. 
Typical implementation of such approaches is to store the key in silicon-based memory devices, which can be prone to physical attacks. 
There have been several approaches to prevent such attacks through hardware primitives such as obfuscation i.e. hiding data in complex chip layouts or below dense metal structures for visual obscurity. 
Recent efforts have, however, shifted to leveraging the inherent randomness induced in silicon devices during the manufacturing process as the secret key, opposed to the traditional binary key stored in silicon devices. Such approaches, called Physically Unclonable Functions (PUFs), have helped provide higher level of security against direct physical attacks alleviate the need for costly physical protection measures.
PUFs have become increasingly popular and have been used in a variety of hardware-based security tasks such as for identification and authentication \cite{Pappu2026}, digital rights management  \cite{Gassend:2002}, bit-commitment protocol \cite{Pappu2026}, and secure multi-party communication \cite{Ruhrmairmulti}. 

Given their natural affinity and subsequent success in providing the secret ``\textit{key}'', recent efforts have focused on showing that the ``unclonable'' and ``unpredictable'' PUFs are vulnerable to crypt-analysis. Common modes of crypt-analyses include side-channel attacks\cite{cryptoeprint:2013:632, cryptoeprint:2013:851}, machine-learning (ML) attacks\cite{Ruhrmair2010} and software attacks, for example, worms and viruses \cite{stallings2012computer}. 
However, current approaches to attacking a PUF architecture make atleast one of two primary assumptions - (1) the underlying PUF architecture is known to the attacker and (2) the PUF can be physically accessed to ``observe'' the signals (such as the noise between interconnects in the circuit). This assumption follows the basic definition in classical cryptography,  Kerckhoffs's principle: ``\textit{A cryptosystem should be secure even if everything about the system, except the key, is public knowledge}''. 

Advances in machine learning have led to a vast majority of the non-invasive attacks explored. Machine learning-based approaches can be characterized by the application of a learned mathematical model on a collected subset of valid challenge-response pairs (CRPs). 
The curation of such data is typically assumed to be an eavesdropping protocol, which is not an unreasonable assumption. 
Hence, CRPs, unique to a PUF architecture, bring both challenges and opportunities. 
Prior works, especially the pioneering work of R\"{u}hmair et al\cite{Ruhrmair2010}, have shown great success in cloning PUFs, gaining cloning accuracy of upto 99.99\%. 
The success of machine learning models in cloning a PUF structure, does come with a caveat - the underlying architecture must be known a-priori.
Given the different types of PUFs that have been proposed and their design variations, gleaning the underlying architecture of a given PUF is not a trivial task, especially in a non-invasive setting. 

To overcome such inhibitions, we focus on an architecture-independent attack, that assumes no prior knowledge of the PUF architecture in the system.
We show that observed CRPs are sufficient to improve cloning accuracy of a strong PUF irrespective of the PUF model while PUF implements the authentication protocol. The attack can simulate PUF network without knowing underlying PUF architecture. 
To evaluate the effectiveness of our approach, we compare against a brute force attack model that leverages the current advances in PUF-architecture cloning. To employ architecture-specific cloning, such as those proposed by \cite{Ruhrmair2010}, we first need to identify the PUF architecture. 
We introduce a mathematical model to use the PUF's response to identify its underlying architecture and then employ the cloning models to attack the PUF. We compute the prediction accuracy of the model by combining the architecture classification accuracy and the cloning accuracy in a harmonic mean. 
The approach is explained in detail in Section \ref{sec:BruteForce}. 
However, in a \textit{controlled PUF}\cite{Gassend:2002}, both machine learning-based attack models cannot be a viable approach as the challenge-response of the underlying PUF is not directly accessible, but is rather protected by a controlling logic interface. 
All challenges are pre-processed by the controlling logic before they are input to the PUF and all responses of the PUF is post processed, adding a level of complexity to the security of the PUF.

To defend against machine learning attacks, we also propose a machine learning-based defense, a \textit{discriminator}, to identify the possibility of cloning using any ML-based attack non-invasive attack. 
Prior approaches to ML-based cloning countermeasures provided added security through obfuscation \cite{8031539,7457162}, meta-algorithms based machine learning \cite{7495550}, and sub-string matching \cite{6714458}. 
However, these countermeasure methods are based on creating complex PUF architectures. 
As we enter into more realizable and immersible Internet of Things (IoT) ecosystem, increasingly complex PUF architectures may not suitable for lightweight IoT systems (e.g., smart cards, sensors, edge devices, etc.).
Hence, we propose a lightweight, probabilistic identification of cloning through machine learning. 

In short, our paper makes the following novel contributions:
\begin{itemize}
\item propose a non-invasive, architecture independent cloning attack on string PUFs,
\item show that a brute force attack on strong PUFs to identify the PUF architecture for cloning is increasingly complex and hence not trivial for feasible cloning, and
\item propose a probabilistic, discriminator model bolster the security of the CRP protocol by identifying possible instances of cloning attacks.
\end{itemize}
To the best of authors' knowledge, this is the first such framework of CRP evaluation on cloned PUFs and its ability to differentiate original PUFs from cloned ones. As such, the techniques discussed in this paper can be applied to a wide variety of PUFs. 

The rest of this paper is organized as follows. Section \ref{sec:ref} briefly reviews related works of machine learning attack and defense mechanisms of strong PUFs. A brute force attack is introduced and evaluated in Section \ref{sec:BruteForce}. The proposed attack method and discriminator model are introduced in Section \ref{sec:approach},
and implementation techniques are presented in Section \ref{sec:implmentation} following experimental evaluation of the proposed approach in Section \ref{sec:results}. Finally,
we conclude with discussion on the feasbility of the proposed approach in Section \ref{sec:conclusions}.


==> 1_introbk.tex <==
\section{Introduction}

% What is the issue
% What has been done
% What you are doing
% Your Contributions
% The roadmap




% What is PUF?
Physically Unclonable Functions (PUFs), a kind of electronic device fingerprint, have recently appeared as a form of identification and authentication \cite{Pappu2026}, digital rights management  \cite{Gassend:2002}, bit-commitment protocol \cite{Pappu2026}, and secure multi-party communication \cite{Ruhrmairmulti}. 
PUFs exploit intrinsic non-reproducible manufacturing variations in an integrated circuit as a ``seed'' for randomness, and can provide low-cost, tamper-evident, and key-storage-free security. 
Different PUF architectures have been proposed in the literature due to the limitations of current Non-Volatile Memory (NVM) based key storage (e.g. easy derivation, simple read-out mechanism, etc.). 
A PUF works by producing a response to an external stimulus (challenge, $c$) and generating an associated unpredictable response (bit/binary string, $r$) for the authentication protocol. These Challenge-Response Pairs (CRPs) form the PUF signature.

% What are ML attack on PUF?
Since the pioneering work by Gassend \emph{et al.} in 2002, PUF design has undergone several variations depending on the number of CRPs to broaden the key generation, storage, and retrieval techniques. 
Although construction of PUF architectures have enabled designers alternatively to apply versatile security to their designs, recent studies have shown the ``unclonable'' and ``unpredictable'' PUFs are vulnerable to cryptanalysis. 
Such cryptanalysis includes side-channel attacks, machine-learning (ML) attacks, software attacks, for example, worms and viruses \cite{stallings2012computer}. 
Ideally, ML-based attacks comprise most of the non-invasive attacks studied so far. To approximate PUFs behavior, attackers can employ simple yet efficient mathematical/numerical models on the eavesdropped CRPs. 
This problem becomes worse when attackers impersonate a PUF by cloning or mimicking its functionality and/or architecture. 
Hence, CRPs, unique to a PUF architecture, bring both challenges and opportunities. 
In this paper, we focus on an architecture-independent attack, that assumes no prior knowledge of the PUF architecture in the system, as well as a defense against this kind of broad attack.
%In this paper, we focus on the ``PUF cloning'' problem in which the proposed ML model can differentiate the original and cloned PUFs given CRPs following an attack scenario.

% Snippet of previous work
Despite improvements in PUF architectures against ML-based attacks, the capabilities of ML modeling attacks have also grown. 
Diverse machine learning techniques, including Logistic Regression (LR), Support Vector Machines (SVMs), Neural Network (NN), Random Forest (RF), and Evaluation Strategies (ES) can be leveraged to clone or mimic PUF behavior.  
R\"{u}hrmair \emph{et al.} first proposed that strong PUF could be cloned using these modeling techniques \cite{Ruhrmair2010,6587277}. The proposed method applied widely-used ML techniques and learned a representative subspace from the CRPs and produced indistinguishable (cloned) PUFs up to a given size and complexity of original PUF architecture. An extension had been developed for PUF modeling attack based on silicon data, which demonstrate that the silicon CRPs conforms to analytical simulation data \cite{6587277}. Physical cloning of SRAM PUFs has been proposed using Focused Ion Beam Circuit Edit  \cite{6581556}. 

Previous ML driven attacks are based on the assumption that the PUF architectures are known {\em a priori}. R\"{u}hrmair \emph{et al.} \cite{Ruhrmair2010} showed that cloning was successful with an prediction rate of 99\%.  In other words, for a successful operation of the cloned PUF, attackers should have some in-depth knowledge about PUF parameters (\#stages, \#XORs, \#MUXs etc.). The limitation of these approaches is that they lack the robustness of attack when the PUF architecture is unknown to create indistinguishable PUF nearby at fine resolution. To guard against ML attacks, researchers have also proposed a number of countermeasures based on obfuscation \cite{8031539,7457162}, meta-algorithms based machine learning \cite{7495550}, and sub-string matching \cite{6714458}. However, these countermeasure methods are based on creating complex PUF architectures. As we are entering into more realizable and immersible Internet of Things (IoT) ecosystem, increasingly complex PUF architectures may not suitable for lightweight IoT systems (e.g., smart cards, sensors, edge devices, etc.).
Moreover, the attacker can mimic the PUF behavior without physically replicating PUF.



% Snippet of this work
% Discriminator model (brief)?
To overcome such inhibitions, this work demonstrates that an architecture-independent adversarial attack on a general strong PUF is feasible. We propose that observed CRPs are sufficient to improve cloning accuracy of a strong PUF irrespective of the PUF model while PUF implements the authentication protocol. The attack can simulate PUF network without knowing underlying PUF architecture. In order to defend such an attack, we introduce a defense model called the discriminator model (DM) as a classifier to distinguish between original and cloned PUF.  The discriminator decides whether each instance of CRP it receives belongs to the actual training dataset or not (attacker induced). It can also effectively defend against the attacks such as modified CRPs and raise alarm once an attack occurs. Another benefit of DM is the improved reliability of PUF architecture. For example, when an attacker applies arbitrary challenges that do not belong to original CRPs to a PUF multiple times, PUF reliability becomes a major concern \cite{Ruhrmair2010}. Hence, it is important to improve the quality of CRPs for PUF reliability. We assume the underlying PUF construction is CMOS-based while the techniques in this paper are scalable for nano-electronics (e.g., memristors, CNT, graphene, etc.) PUF architectures as well. 

% Summary of the paper

In short, our paper makes the following novel contributions:
\begin{itemize}

\item Formulate a PUF architecture independent attack approach that can clone a strong PUF by eavesdropping CPRs  with zero-knowledge of the underlying PUF architecture;
%with observed CRPs yields maximizing cloneable PUF performance.
%Formulate a PUF-agnostic attack approach which can determine the efficiency of  the cloned PUF with zero-knowledge of the underlying PUF architecture;
%with observed CRPs yields maximizing cloneable PUF performance.

\item We also propose a discriminator model to distinguish between original and attacker induced CRPs without sacrificing PUF reliability.

% When attackers use the fake CRPs 
% to learn the underlying PUF behavior, our proposed discriminator model can distinguish between original and fake CRPs.
\end{itemize}

To the best of authors' knowledge, this is the first such framework of CRP evaluation on cloned PUFs and it can differentiate original PUFs from cloned ones. As such, the techniques discussed in this paper can be applied to a wide variety of PUFs. 

The rest of this paper is organized as follows. Section \ref{sec:ref} briefly reviews related works of machine learning attack and defense mechanisms of strong PUFs. The proposed attack method and discriminator model are introduced in Section \ref{sec:approach},
and implementation techniques are presented in  Section \ref{sec:implmentation}  following experimental results in Section \ref{sec:results}. Finally,
we conclude the paper in Section \ref{sec:conclusions}.



% Why do we care about this problem and the results?
% • Importance of the work,
% • Difficulty of the area
% • Impact it has if successful




==> reviews.tex <==
Reviewer 1:
The paper propose an attack for PUF which has no assumption about the PUF underlying architecture. They explain how machine learning technique can be used to discriminate PUFs before launching a classical attack. 
* a whole paragraph in bold font -DOne
* several typos ("architecture may not suitable for" for instance) - Done
* The paper is very difficult to read anyway - Done

Reviewer 2:

The paper is overall well written. The research objectives of the work are clear, and the argument is substantiated and credible. The proposed scheme has strong feasibility and practical application prospects. The reviewer has the following questions and suggestions:

*  The staged attack model is mentioned in this paper: the two-stage attack model in the section III and the three-stage attack model in the section V. However, it is not clear how these staged attack models work. It is highly suggested to elaborate more about this background. - done

* In the section V, only experimental results are presented. It is highly suggested to analyze and discuss more about the underlying reasons behind the results - Done

*  The proposed attack and prediction techniques target strong PUF. Are the techniques still applicable to weak PUF? - Done


REVIEW 3
The authors propose to use machine learning based methods to attack the PUF based security mechanism on IoT devices. If a certain amount of challenge and response pairs are obtained, the underlying stochastic function of specific PUF architecture could be identified after training. In addition, a countermeasure is introduced to identify the clone. The results show that almost all types of strong PUFs could be cloned with high accuracy, and all the clones could be detected efficiently as well.

1)      The PUF based authentication procedure depicted by the authors is reasonable, but it is not clear why and how a strong PUF would be used on a resource constrained IoT devices:
      a) The reviewer is unaware of any applications that implement strong PUF on IoT node devices. Is it worth and practical to implement a strong PUF on a tiny sensor which only costs a few dollar? - ??
     b) The CRPs of strong PUFs need be stored in a secure server. Retrieving of all the stored data from the secure server to the authentication site, may cause additional security problems. It is also not clear who will maintain that secure server as there are hundreds (possibly thousands) of different IoT device vendors. 

2)      There is no physical implementation in this paper. 
    a)How the PUFs are implemented and emulated? What is the difference in the training data between different architectures? - Done
    
    b)Although 800 CSPs are collected for each architecture, it is still confusing that whether the model could be applied widely. For example, 800 pairs are collected from eavesdropping device A, then a model is created and tested. How could we know this model would also be valid for device B, C, D even they are all same architecture? In this case, does it mean for each device, a certain amount of CSPs must be known? If so, what is this amount, 800? If not, how could it be proved?-???

3)      It is still confusing that how the countermeasure “Discriminator” works. The results show that PUF architectures could be cloned with an average error 10. It proves the attack is possible. However, it is reasonable to consider the aging of the devices. The response of a challenge should always allow some errors exist. How could you determine whether the error is from a malicious clone device or a benign aged device? - done

4)  Why the Discriminator Error decreases while the PUF complexity and cloning error increasing? - done

5)  The overall contribution of this work is limited, the only convincible novel point is that this method eliminates the need of brute force attack on the PUF architecture. However, as the authors have mentioned, the security of PUF does not rely on hiding the architecture but relies on the stochastic nature of the PUF. The procedure of hiding/knowing the architecture is not the most significant factor of the attack at all.

6) There are quite a few grammatical errors and typos. - Done


REVIEW 4
----------- Overall evaluation -----------
The authors proposed a brute-force attack to clone the PUF architectures, wherein they took the of an ML model. They evaluated the effectiveness of the proposed technique by considering several strong PUF architectures. Their model is architecture independent and provides decent results.
* No comments mentioned
